The DynAlloy Visualizer

We present an extension to the DynAlloy tool to navigate DynAlloy counterexamples: the DynAlloy Visualizer. The user interface mimics the functionality of a programming language debugger. Without this tool, a DynAlloy user is forced to deal with the internals of the Alloy intermediate representation in order to debug a flaw in her model.

==> eptcsdata.tex <==
\providecommand{\firstpage}{59}
\providecommand{\publicationstatus}{Nazareno Aguirre, Leila Ribeiro (Eds.):\\
First Latin American Workshop on Formal Methods (LAFM 2013)\\
EPTCS 139, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.139.6}{10.4204/EPTCS.139.6}}
\pdfoutput=1

